Road Mapping and Localization using Sparse Semantic Visual Features

We present a novel method for visual mapping and localization for autonomous vehicles, by extracting, modeling, and optimizing semantic road elements. Specifically, our method integrates cascaded deep models to detect standardized road elements instead of traditional point features, to seek for improved pose accuracy and map representation compactness. To utilize the structural features, we model road lights and signs by their representative deep keypoints for skeleton and boundary, and parameterize lanes via piecewise cubic splines. Based on the road semantic features, we build a complete pipeline for mapping and localization, which includes a) image processing front-end, b) sensor fusion strategies, and c) optimization backend. Experiments on public datasets and our testing platform have demonstrated the effectiveness and advantages of our method by outperforming traditional approaches.

==> sec2_related_works.tex <==
\section{Related Works}
\label{sec:rel}

The backbone of recent adaptable multi-sensor visual SLAM systems~\cite{cadena2016past,mur2017orb,qin2018vins,schneider2018maplab,chen2019perception} is a tightly-coupled state optimization framework with sliding window strategies. Local visual features are extracted and tracked in the front-end, and then triangulated and optimized with trajectories and other proprioceptive sensor measurements in the back-end. The triangulated landmarks can be serialized to form a visual localization map for online map-aided localization.
As such, reliable state optimization constraints can be fixed, and cumulative drift can be fixed accordingly. Based on this backbone, geometry and vision researchers propose a variety of algorithms to enhance its components.

\textbf{Deep perception for SLAM.} 
% Description and Matching.
Several deep models have been proposed recently to replace handcrafted local features~\cite{lowe2004distinctive,rublee2011orb} during extraction, description, and matching respectively.
SuperPoints~\cite{detone2018superpoint} and SEKD~\cite{song2020sekd} intend to extract invariant features by rejecting the ones extracted on moving instances, which are not suitable for positioning. SuperGlue~\cite{wang2019superglue} constructs associations between these features among different frames.

% Segmentation and its practical issues on restricted computing resources.
Towards the instance level perception, advanced systems based on stereo~\cite{barsan2018robust} or RGB-D~\cite{runz2018maskfusion} cameras propose to use segmentation networks~\cite{he2017mask} and reconstruct scene instances as dense meshes.
% Detection.
Compared to these segmentation networks, detection networks~\cite{zhou2019objects} are relatively lightweight for embedded platforms. Hence, some monocular SLAM systems propose to use detected results for estimating the coarse location of instances~\cite{yang2019cubeslam}, or simply labeling instance-wise semantic types to filter geometrical matching~\cite{bowman2017probabilistic}.
% Cascaded detection + skeleton.
Derived from these detection networks, we propose to cascadingly perform supervised keypoint extraction in these detected instances. This process is not only feasible for standardized road elements, but also capable of providing more detailed geometrical structures as well as point-wise semantic labels for localization.

\textbf{Parameterization of map primitives.}
% Multi-view geometry.
In multi-view geometry, recent works attempt to discover new parameterization strategies for primitives beyond 3D points~\cite{mur2017orb}.
% Lines and planes.
Some methods focus on lines~\cite{gomez2019pl} extracted by edge detection methods~\cite{von2008lsd} or deep models~\cite{Sun2019SemLSD}, and some represent walls and grounds by Manhattan~\cite{yang2016pop} or general~\cite{kaess2015simultaneous,yang2019monocular} planes.
% Objects and curves.
A few works also try to parameterize detected bounding boxes as cuboids~\cite{yang2019cubeslam} or quadratics~\cite{nicholson2018quadricslam}, and lanes as splines~\cite{wang2018fully,rao2012curveslam}.

% Relations with deep models.
Similar to feature points, a highly accurate reconstruction of these 3D entities requires precise 2D extraction on images to perform a maximum-a-posterior triangulation. Hence, given output keypoints from neural networks, we need to additionally assess their pixel accuracy, which guides the setting of measurement uncertainty during state estimation. Following such a strategy, we introduce a novel method in our system to reconstruct road lanes as piecewise cubic Catmull-Rom splines. While for cascadingly detected structural road objects, we notice that triangulating geometrically meaningful deep keypoints, e.g., skeleton and polygon of instances, is beneficial for localization.

\textbf{Localization with maps.} In modern localization applications, maps are often constructed with high-end sensors and sufficient computations, to ensure trajectory correctness and landmark quality. A variety of 2D-2D methods propose to describe frames using descriptor-based representations, e.g., DBoW2~\cite{galvez2012bags} or VLAD~\cite{arandjelovic2016netvlad}, for efficient frame-to-frame matching. Landmark-based algorithms tend to use frame-to-map registration (or submap-to-map~\cite{jeong2017road} conveying more information) for obtaining reliable geometrical matching hints. In order to integrate the semantic information into localization systems, some approaches~\cite{toft2018semantic,shi2019visual} use segmentation networks to classify feature points with semantic types, so as to perform scoring on 2D-3D matches. Similarly, 3D-3D matching use ground coefficients~\cite{qin2020avp,jeong2017road} or directly employ RGB-D cameras~\cite{liu2019global} to get a dense point cloud for performing label-aided iterative closest point registrations~\cite{segal2009generalized}. Besides, a few approaches~\cite{schonberger2018semantic} propose to learn semantic representations from volumetric maps via deep networks. Still, they need dense depth maps and sufficient computing resources.

Unlike the above methods, detected representative keypoints for objects in our reconstructed semantic maps are directly triangulated. Thus they are sparse (i.e., about 400 points per kilometer on roads) and highly distinguishable (i.e., the density of same-label points remains the same as their instance level). In such a case, a label-aware perspective-n-point algorithm, which is both efficient on sparse points and free from initial guesses, can outperform both frame-to-frame query and dense frame-to-map registration methods in a lightweight manner.

